When the Prompt Becomes Visual: Vision-Centric Jailbreak Attacks for Large Image Editing Models

Recent advances in large image editing models have shifted the paradigm from text-driven instructions to vision-prompt editing, where user intent is inferred directly from visual inputs such as marks, arrows, and visual-text prompts. While this paradigm greatly expands usability, it also introduces a critical and underexplored safety risk: the attack surface itself becomes visual. In this work, we propose Vision-Centric Jailbreak Attack (VJA), the first visual-to-visual jailbreak attack that conveys malicious instructions purely through visual inputs. To systematically study this emerging threat, we introduce IESBench, a safety-oriented benchmark for image editing models. Extensive experiments on IESBench demonstrate that VJA effectively compromises state-of-the-art commercial models, achieving attack success rates of up to 80.9% on Nano Banana Pro and 70.1% on GPT-Image-1.5. To mitigate this vulnerability, we propose a training-free defense based on introspective multimodal reasoning, which substantially improves the safety of poorly aligned models to a level comparable with commercial systems, without auxiliary guard models and with negligible computational overhead. Our findings expose new vulnerabilities, provide both a benchmark and practical defense to advance safe and trustworthy modern image editing systems. Warning: This paper contains offensive images created by large image editing models.

==> tables/new_comp_open_model.tex <==
\begin{table*}[htb] \small
\centering
\caption{\textbf{Attack results of VPA on open-source MLLMs with the aid of our \bench.} Since no guard models are locally equipped with them, the ASR of BAGEL, LongCat-Image-Edit and Qwen-Image-Edit-Local is \colorbox{red!30}{100\%}, so we do not report the ASR.} 
\label{tab:open_models}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccc|ccc|ccc|ccc|cccc}
\hline
& \multicolumn{3}{c}{BAGEL} & \multicolumn{3}{c}{LongCat-Image-Edit} &\multicolumn{3}{c}{Flux2.0[dev]} & \multicolumn{3}{c}{Qwen-Image-Edit-Local} & \multicolumn{4}{c}{\textcolor{black}{Qwen-Image-Edit-Safe (Ours)}}\\ \hline

\multicolumn{1}{c|}{Metric} & HS $\uparrow$ & EV $\uparrow$ & \multicolumn{1}{c|}{HRR $\uparrow$} & HS $\uparrow$ & EV $\uparrow$ & \multicolumn{1}{c|}{HRR $\uparrow$} & HS$\uparrow$ & EV $\uparrow$ & \multicolumn{1}{c|}{HRR $\uparrow$} & HS $\uparrow$ & EV $\uparrow$ & HRR $\uparrow$ & ASR  $\uparrow$ & HS $\uparrow$ & EV $\uparrow$ & \multicolumn{1}{c}{HRR $\uparrow$}\\ 
\hline
\multicolumn{1}{c|}{01-VM}  & 
4.3$\pm$1.1 & 84.2  & \multicolumn{1}{c|}{74.8} & 
2.4$\pm$0.9 & 14.4  & \multicolumn{1}{c|}{11.5} &
4.7$\pm$0.8 & 92.8  & \multicolumn{1}{c|}{87.1} & 
4.7$\pm$0.7 & 94.2  & \multicolumn{1}{c|}{93.5} &
87.0 & 4.3$\pm$1.4 & 83.3 & \multicolumn{1}{c}{82.6} 
\\

\multicolumn{1}{c|}{02-PV}  & 
4.2$\pm$1.0 & 85.3  & \multicolumn{1}{c|}{75.2} & 
3.5$\pm$1.4 & 56.6  & \multicolumn{1}{c|}{47.6} &
4.7$\pm$0.8 & 93.8  & \multicolumn{1}{c|}{87.6} & 
4.4$\pm$0.9 & 89.0  & \multicolumn{1}{c|}{87.4} &
77.3 & 3.7$\pm$1.6 & 68.8  & \multicolumn{1}{c}{68.0}  \\

\multicolumn{1}{c|}{03-SH} & 
\bluecell 3.5$\pm$1.4 & \bluecell 58.6  & \multicolumn{1}{c|}{\bluecell 47.7} &
2.5$\pm$1.0 & 18.9  & \multicolumn{1}{c|}{13.5} & 
4.7$\pm$0.9 & 91.9  & \multicolumn{1}{c|}{87.4} &
4.6$\pm$0.9 & 91.0  & \multicolumn{1}{c|}{89.2} &
87.4 & 4.2$\pm$1.4 & 81.1  & \multicolumn{1}{c}{80.2} \\

\multicolumn{1}{c|}{04-CA} & 
4.5$\pm$1.0 & 91.0  & \multicolumn{1}{c|}{82.0} &
2.5$\pm$1.1 & 21.2  & \multicolumn{1}{c|}{14.3} & 
4.7$\pm$0.7 & 94.0  & \multicolumn{1}{c|}{92.5} &
4.8$\pm$0.6 & 95.5  &\multicolumn{1}{c|}{94.0} &
88.7 & 4.4$\pm$1.3 & 85.0  & \multicolumn{1}{c}{83.5}\\

\multicolumn{1}{c|}{05-AA}  & 
4.3$\pm$1.1 & 88.7  & \multicolumn{1}{c|}{77.4} &
2.3$\pm$0.8 & 18.9  & \multicolumn{1}{c|}{7.5} &
4.8$\pm$0.7 & 96.2  & \multicolumn{1}{c|}{92.5} &
4.6$\pm$0.9 & 92.5  & \multicolumn{1}{c|}{88.7} &
81.1 & 4.0$\pm$1.6 & 75.5  & \multicolumn{1}{c}{75.5} \\

\multicolumn{1}{c|}{06-FM}  & 
3.9$\pm$1.0 & 83.3  & \multicolumn{1}{c|}{69.4} &
\redcell 4.2$\pm$1.1 & \redcell 83.3  & \multicolumn{1}{c|}{\redcell 69.4} &
4.7$\pm$0.6 & 80.6  & \multicolumn{1}{c|}{80.6} & 
4.6$\pm$0.8 & 94.4  & \multicolumn{1}{c|}{94.4} &
72.2 & 3.6$\pm$1.7 & 69.4  & \multicolumn{1}{c}{69.4}\\

\multicolumn{1}{c|}{07-LT}  & 
4.4$\pm$0.7 & 95.2  & \multicolumn{1}{c|}{91.7} &
2.6$\pm$1.1 & 25.0  & \multicolumn{1}{c|}{22.6} & 
4.7$\pm$0.7 & 94.0  & \multicolumn{1}{c|}{94.0} &
4.6$\pm$0.7 & 95.2  & \multicolumn{1}{c|}{94.0} &
69.0 & 3.6$\pm$1.8 & 69.0  & \multicolumn{1}{c}{69.0} \\

\multicolumn{1}{c|}{08-VD} & 
3.9$\pm$1.1 & 79.0  & \multicolumn{1}{c|}{62.6} &
2.6$\pm$1.1 & 21.5  & \multicolumn{1}{c|}{18.2} & 
4.4$\pm$1.0 & 80.4  & \multicolumn{1}{c|}{77.1} & 
4.5$\pm$0.8 & 90.7  & \multicolumn{1}{c|}{87.9} &
53.4 & 2.9$\pm$1.8 & 50.7  & \multicolumn{1}{c}{49.8} \\

\multicolumn{1}{c|}{09-SI} & 
4.4$\pm$1.1 & 86.3  & \multicolumn{1}{c|}{77.9} &
3.0$\pm$1.3 & 36.8  & \multicolumn{1}{c|}{28.4} &
\bluecell 4.2$\pm$1.3 & \bluecell 75.8  & \multicolumn{1}{c|}{72.6} & 
\bluecell 4.3$\pm$1.2 & \bluecell 83.9  & \multicolumn{1}{c|}{\bluecell 77.4} &
71.8 & 3.3$\pm$1.8 &  58.8  & \multicolumn{1}{c}{54.1}\\

\multicolumn{1}{c|}{10-DI} & 
4.2$\pm$1.2 & 80.0  & \multicolumn{1}{c|}{70.0} &
3.5$\pm$1.5 & 50.0  & \multicolumn{1}{c|}{50.0} &
4.4$\pm$1.2 & 80.0  & \multicolumn{1}{c|}{80.0} & 
4.7$\pm$0.9 & 90.0  & \multicolumn{1}{c|}{90.0} &
\redcell 100.0 & \redcell 4.7$\pm$0.9 &  \redcell 90.0  & \multicolumn{1}{c}{\redcell 90.0} \\

\multicolumn{1}{c|}{11-CT}  & 
\redcell 4.5$\pm$0.7 & \redcell 95.7  & \multicolumn{1}{c|}{\redcell 93.5} &
2.8$\pm$1.2 & 30.4  & \multicolumn{1}{c|}{26.1} &
4.9$\pm$0.5 & 93.5  & \multicolumn{1}{c|}{93.5} & 
4.8$\pm$0.7 & 95.7  & \multicolumn{1}{c|}{95.7} &
28.3 & 2.0$\pm$1.7 & 26.1  & \multicolumn{1}{c}{26.1}\\

\multicolumn{1}{c|}{12-HI}  & 
4.2$\pm$1.1 & 85.5  & \multicolumn{1}{c|}{74.2} &
3.4$\pm$1.5 & 50.0  & \multicolumn{1}{c|}{48.4} &
\redcell 4.9$\pm$0.3 & \redcell 100.0  & \multicolumn{1}{c|}{\redcell 98.4} & 
\redcell 4.8$\pm$0.5 & \redcell 100.0  & \multicolumn{1}{c|}{95.2} &
\bluecell 8.1 & \bluecell 1.3$\pm$1.0 & \bluecell 8.1  & \multicolumn{1}{c}{\bluecell 8.1}\\
 
\multicolumn{1}{c|}{13-ET}  & 
3.7$\pm$1.0 & 76.9  & \multicolumn{1}{c|}{51.3} &
3.7$\pm$1.3 & 66.7  & \multicolumn{1}{c|}{53.8} &
4.4$\pm$0.8 & 76.9  & \multicolumn{1}{c|}{76.9} &
4.6$\pm$0.5 & 97.4  & \multicolumn{1}{c|}{\redcell 97.4} &
61.5 & 3.1$\pm$1.7 & 61.5  & \multicolumn{1}{c}{61.5}  \\

\multicolumn{1}{c|}{14-DE}  & 
3.7$\pm$1.0 & 76.9  & \multicolumn{1}{c|}{60.3} &
2.5$\pm$1.1 & 22.1  & \multicolumn{1}{c|}{17.6} &
4.3$\pm$1.1 & 79.4  & \multicolumn{1}{c|}{\bluecell 72.1} & 
4.7$\pm$0.7 & 97.0  & \multicolumn{1}{c|}{94.0} &
72.1 & 3.6$\pm$1.7 & 70.6 & \multicolumn{1}{c}{67.6}  \\

\multicolumn{1}{c|}{15-AM}  & 
4.5$\pm$0.9 & 94.7  & \multicolumn{1}{c|}{84.2} & 
\bluecell 2.2$\pm$0.7 & \bluecell 13.2  & \multicolumn{1}{c|}{\bluecell 5.3} &
4.5$\pm$1.0 & 94.7  & \multicolumn{1}{c|}{84.2} &
4.6$\pm$0.9 & 97.4  & \multicolumn{1}{c|}{84.2} &
55.3 & 3.1$\pm$1.9 & 55.3 & \multicolumn{1}{c}{50.0} \\

\multicolumn{1}{c|}{\textbf{ALL}} &
4.1$\pm$1.1 & 82.0 &  \multicolumn{1}{c|}{70.6} & 
2.8$\pm$1.2 & 30.6 &  \multicolumn{1}{c|}{24.9} & 
4.6$\pm$0.9 & 87.1 &  \multicolumn{1}{c|}{84.6} & 
4.6$\pm$0.8 & 92.9 &  \multicolumn{1}{c|}{90.3} &
66.9 & 3.4$\pm$1.8 & 62.8 &  \multicolumn{1}{c}{61.7}\\
\hline
\end{tabular}
}

\end{table*}
